Tricking LLMs into Disobedience: Formalizing, Analyzing, and Detecting Jailbreaks

Recent explorations with commercial Large Language Models (LLMs) have shown that non-expert users can jailbreak LLMs by simply manipulating their prompts; resulting in degenerate output behavior, privacy and security breaches, offensive outputs, and violations of content regulator policies. Limited studies have been conducted to formalize and analyze these attacks and their mitigations. We bridge this gap by proposing a formalism and a taxonomy of known (and possible) jailbreaks. We survey existing jailbreak methods and their effectiveness on open-source and commercial LLMs (such as GPT-based models, OPT, BLOOM, and FLAN-T5-XXL). We further discuss the challenges of jailbreak detection in terms of their effectiveness against known attacks. For further analysis, we release a dataset of model outputs across 3700 jailbreak prompts over 4 tasks.

==> tables/manual_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|ll|ll|ll|ll|}
\hline
                                     & Model                                              & \multicolumn{2}{l|}{code-davinci-002}                                   & \multicolumn{2}{l|}{FLAN}                                               & \multicolumn{2}{l|}{gpt-3.5-turbo}                                      & \multicolumn{2}{l|}{OPT}                                                \\ \hline
\multirow{2}{*}{Task}                & \multirow{2}{*}{\backslashbox[20mm]{Prog.}{GPT-4}} & \multicolumn{1}{l|}{\multirow{2}{*}{Agree}} & \multirow{2}{*}{Disagree} & \multicolumn{1}{l|}{\multirow{2}{*}{Agree}} & \multirow{2}{*}{Disagree} & \multicolumn{1}{l|}{\multirow{2}{*}{Agree}} & \multirow{2}{*}{Disagree} & \multicolumn{1}{l|}{\multirow{2}{*}{Agree}} & \multirow{2}{*}{Disagree} \\
                                     &                                                    & \multicolumn{1}{l|}{}                       &                           & \multicolumn{1}{l|}{}                       &                           & \multicolumn{1}{l|}{}                       &                           & \multicolumn{1}{l|}{}                       &                           \\ \hline
Code generation                      & Agree                                              & \multicolumn{1}{l|}{7}                      & 2                         & \multicolumn{1}{l|}{8}                      & 5                         & \multicolumn{1}{l|}{20}                     & 9                         & \multicolumn{1}{l|}{19}                     & 10                        \\ \hline
                                     & Disagree                                           & \multicolumn{1}{l|}{12}                     & 29                        & \multicolumn{1}{l|}{2}                      & 35                        & \multicolumn{1}{l|}{6}                      & 9                         & \multicolumn{1}{l|}{9}                      & 12                        \\ \hline
\multirow{2}{*}{Summarization}       & Agree                                              & \multicolumn{1}{l|}{32}                     & 4                         & \multicolumn{1}{l|}{9}                      & 6                         & \multicolumn{1}{l|}{24}                     & 5                         & \multicolumn{1}{l|}{28}                     & 0                         \\ \cline{2-10} 
                                     & Disagree                                           & \multicolumn{1}{l|}{7}                      & 7                         & \multicolumn{1}{l|}{17}                     & 18                        & \multicolumn{1}{l|}{13}                     & 8                         & \multicolumn{1}{l|}{6}                      & 16                        \\ \hline
\multirow{2}{*}{Text classification} & Agree                                              & \multicolumn{1}{l|}{10}                     & 7                         & \multicolumn{1}{l|}{13}                     & 8                         & \multicolumn{1}{l|}{13}                     & 21                        & \multicolumn{1}{l|}{43}                     & 1                         \\ \cline{2-10} 
                                     & Disagree                                           & \multicolumn{1}{l|}{24}                     & 9                         & \multicolumn{1}{l|}{21}                     & 8                         & \multicolumn{1}{l|}{14}                     & 2                         & \multicolumn{1}{l|}{4}                      & 2                         \\ \hline
\multirow{2}{*}{Translation}         & Agree                                              & \multicolumn{1}{l|}{37}                     & 4                         & \multicolumn{1}{l|}{22}                     & 18                        & \multicolumn{1}{l|}{38}                     & 3                         & \multicolumn{1}{l|}{25}                     & 11                        \\ \cline{2-10} 
                                     & Disagree                                           & \multicolumn{1}{l|}{7}                      & 2                         & \multicolumn{1}{l|}{6}                      & 4                         & \multicolumn{1}{l|}{2}                      & 7                         & \multicolumn{1}{l|}{6}                      & 8                         \\ \hline
\end{tabular}%
}
\caption{Overall annotator agreement for every model and every task. The horizontal agreement and disagreement numbers represent the number of points that agree or disagree with GPT-4's output. The vertical agreements represent the same for the programmatic property tests.}
\label{tab:annotator_agreement_overall}
\end{table*}
